DORA Explorer: Improving the Exploration Ability of LLMs Without Training

Large language model (LLM) agents for sequential decision-making struggle to produce diverse outputs. This leads to insufficient exploration, suboptimal solutions, and repeated actions. Actions are generated at the sequence level, but existing sampling strategies, such as temperature scaling, introduce diversity at the token level, not at the sequence level. We introduce DORA EXPLORER (Diversity-Oriented Ranking of Actions), a training-free, inference-time algorithm for improving exploration in LLM agents. DORA generates multiple candidate actions, scores them using sequence-level log-probability statistics, and samples an action via a tunable exploration parameter. We first study exploration in the classic Multi-Armed Bandit setting, where DORA substantially outperforms temperature-based sampling. Our main evaluation is on the Text Adventure Learning Environment Suite (TALES), where prompting strategies fail to explore but DORA delivers consistent gains across model families, e.g., 31.43% (ReAct) -> 45.5% (DORA) for Qwen-2.5 7B in TextWorld. Beyond exploration, DORA prevents common failures, such as getting stuck in loops. Our project is available at: https://dora-explore.github.io/.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/TALES_unique_state_visted.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lccc}
\toprule
\textbf{Method} & \textbf{TextWorld} & \textbf{ScienceWorld} & \textbf{AlfWorld} \\
\midrule
Zero-shot & 14.0 & 6.5 & 2.67 \\
Prompt Explore & 12.1 & 8.9 & 3.67 \\
CoT & 17.5 & 8.23 & 3.25 \\
ToT & 12.1 & 4.6 & 3.67 \\
DORA (Auto) & \textbf{32.0} & \textbf{20.23} & \textbf{27.92} \\
\bottomrule
\end{tabular}
\caption{Average number of unique states visited per task in different TALES environments. Higher values indicate the agent got to see more different states and thus had a greater coverage of the environment.}
\label{tab:state_diversity}
\end{table}

==> tables/mabTableV2.tex <==
\begin{table}[h!]
\centering
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.6}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l*{11}{c}}
\toprule
 \multirow{2}{*}{\diagbox[ width=8em, height=3em]{\textbf{Metric}}{\textbf{Method}}} & \multicolumn{4}{c}{Classic Strategies} & \multicolumn{6}{c}{Temperature ($\tau$) Scaling} & \multirow{2}{*}{\textbf{DORA}} \\ \cmidrule(lr){2-5} \cmidrule(lr){6-11}
 & UCB
 & TS
 & Greedy
 & $\varepsilon$-Greedy
 & $\tau=0.0$
 & $\tau=0.3$
 & $\tau=0.7$
 & $\tau=1.0$
 & $\tau=1.5$
 & $\tau=2.0$
 & \textbf{DORA} \\
\midrule

% MeanReward (high = good: green=best, red=worst)
% Values: 0.531, 0.512, 0.506, 0.490, 0.410, 0.410, 0.402, 0.409, 0.488, 0.481, 0.514
% Rank:     1      3      4      5     10     10      11     10      6      7      2
MeanReward
  & \cellcolor[HTML]{27ae60}\textbf{\textcolor{white}{0.53}}
  & \cellcolor[HTML]{a8d96a}\textbf{\textcolor{black}{0.51}}
  & \cellcolor[HTML]{c8e06a}\textbf{\textcolor{black}{0.51}}
  & \cellcolor[HTML]{f1c40f}\textbf{\textcolor{black}{0.49}}
  & \cellcolor[HTML]{e74c3c}\textbf{\textcolor{white}{0.41}}
  & \cellcolor[HTML]{e74c3c}\textbf{\textcolor{white}{0.41}}
  & \cellcolor[HTML]{c0392b}\textbf{\textcolor{white}{0.40}}
  & \cellcolor[HTML]{e74c3c}\textbf{\textcolor{white}{0.41}}
  & \cellcolor[HTML]{f1c40f}\textbf{\textcolor{black}{0.49}}
  & \cellcolor[HTML]{d4ac0d}\textbf{\textcolor{black}{0.48}}
  & \cellcolor[HTML]{82ca60}\textbf{\textcolor{black}{0.51}}
\\

% MedianReward (high = good)
% Values: 0.535, 0.515, 0.520, 0.500, 0.388, 0.388, 0.388, 0.395, 0.508, 0.490, 0.518
% MedianReward
%   & \cellcolor[HTML]{27ae60}\textbf{\textcolor{white}{0.53}}
%   & \cellcolor[HTML]{a8d96a}\textbf{\textcolor{black}{0.51}}
%   & \cellcolor[HTML]{bee06a}\textbf{\textcolor{black}{0.52}}
%   & \cellcolor[HTML]{f1c40f}\textbf{\textcolor{black}{0.50}}
%   & \cellcolor[HTML]{c0392b}\textbf{\textcolor{white}{0.39}}
%   & \cellcolor[HTML]{c0392b}\textbf{\textcolor{white}{0.39}}
%   & \cellcolor[HTML]{c0392b}\textbf{\textcolor{white}{0.39}}
%   & \cellcolor[HTML]{e74c3c}\textbf{\textcolor{white}{0.39}}
%   & \cellcolor[HTML]{d4e56a}\textbf{\textcolor{black}{0.51}}
%   & \cellcolor[HTML]{f1c40f}\textbf{\textcolor{black}{0.49}}
%   & \cellcolor[HTML]{8fd16a}\textbf{\textcolor{black}{0.52}}
% \\

% SuffFailFreq(T/2) (low = good: green=low, red=high)
% Values: 0.02, 0.00, 0.42, 0.30, 0.90, 0.90, 0.95, 0.85, 0.05, 0.00, 0.00
SuffFailFreq($\tau$/2)
  & \cellcolor[HTML]{82ca60}\textbf{\textcolor{black}{0.02}}
  & \cellcolor[HTML]{27ae60}\textbf{\textcolor{white}{0.00}}
  & \cellcolor[HTML]{f1c40f}\textbf{\textcolor{black}{0.42}}
  & \cellcolor[HTML]{d4ac0d}\textbf{\textcolor{black}{0.30}}
  & \cellcolor[HTML]{e74c3c}\textbf{\textcolor{white}{0.90}}
  & \cellcolor[HTML]{e74c3c}\textbf{\textcolor{white}{0.90}}
  & \cellcolor[HTML]{c0392b}\textbf{\textcolor{white}{0.95}}
  & \cellcolor[HTML]{e74c3c}\textbf{\textcolor{white}{0.85}}
  & \cellcolor[HTML]{6cbf60}\textbf{\textcolor{white}{0.05}}
  & \cellcolor[HTML]{27ae60}\textbf{\textcolor{white}{0.00}}
  & \cellcolor[HTML]{27ae60}\textbf{\textcolor{white}{0.00}}
\\

% K*MinFrac (high = good)
% Values: 0.120, 0.220, 0.030, 0.018, 0.000, 0.000, 0.000, 0.000, 0.090, 0.290, 0.292
% K*MinFrac
%   & \cellcolor[HTML]{d4ac0d}\textbf{\textcolor{black}{0.12}}
%   & \cellcolor[HTML]{a8d96a}\textbf{\textcolor{black}{0.22}}
%   & \cellcolor[HTML]{e74c3c}\textbf{\textcolor{white}{0.03}}
%   & \cellcolor[HTML]{e74c3c}\textbf{\textcolor{white}{0.02}}
%   & \cellcolor[HTML]{c0392b}\textbf{\textcolor{white}{0.00}}
%   & \cellcolor[HTML]{c0392b}\textbf{\textcolor{white}{0.00}}
%   & \cellcolor[HTML]{c0392b}\textbf{\textcolor{white}{0.00}}
%   & \cellcolor[HTML]{c0392b}\textbf{\textcolor{white}{0.00}}
%   & \cellcolor[HTML]{f1c40f}\textbf{\textcolor{black}{0.09}}
%   & \cellcolor[HTML]{5cba60}\textbf{\textcolor{white}{0.29}}
%   & \cellcolor[HTML]{27ae60}\textbf{\textcolor{white}{0.29}}
% \\

% BestArmFrac (high = good)
% Values: 0.660, 0.570, 0.530, 0.455, 0.100, 0.100, 0.050, 0.094, 0.440, 0.430, 0.585
BestArmFrac
  & \cellcolor[HTML]{27ae60}\textbf{\textcolor{white}{0.66}}
  & \cellcolor[HTML]{82ca60}\textbf{\textcolor{black}{0.57}}
  & \cellcolor[HTML]{a8d96a}\textbf{\textcolor{black}{0.53}}
  & \cellcolor[HTML]{f1c40f}\textbf{\textcolor{black}{0.45}}
  & \cellcolor[HTML]{e74c3c}\textbf{\textcolor{white}{0.10}}
  & \cellcolor[HTML]{e74c3c}\textbf{\textcolor{white}{0.10}}
  & \cellcolor[HTML]{c0392b}\textbf{\textcolor{white}{0.05}}
  & \cellcolor[HTML]{e74c3c}\textbf{\textcolor{white}{0.09}}
  & \cellcolor[HTML]{d4ac0d}\textbf{\textcolor{black}{0.44}}
  & \cellcolor[HTML]{d4ac0d}\textbf{\textcolor{black}{0.43}}
  & \cellcolor[HTML]{6cbf60}\textbf{\textcolor{black}{0.58}}
\\

% GreedyFrac (low = good: green=low, red=high)
% Values: 0.790, 0.650, 0.990, 0.966, 1.000, ---, ---, ---, ---, ---, 0.635
% GreedyFrac
%   & \cellcolor[HTML]{e74c3c}\textbf{\textcolor{white}{0.79}}
%   & \cellcolor[HTML]{f1c40f}\textbf{\textcolor{black}{0.65}}
%   & \cellcolor[HTML]{c0392b}\textbf{\textcolor{white}{0.99}}
%   & \cellcolor[HTML]{c0392b}\textbf{\textcolor{white}{0.97}}
%   & \cellcolor[HTML]{c0392b}\textbf{\textcolor{white}{1.00}}
%   & \multicolumn{1}{c}{\cellcolor[HTML]{f5f5f5}---}
%   & \multicolumn{1}{c}{---}
%   & \multicolumn{1}{c}{\cellcolor[HTML]{f5f5f5}---}
%   & \multicolumn{1}{c}{---}
%   & \multicolumn{1}{c}{\cellcolor[HTML]{f5f5f5}---}
%   & \cellcolor[HTML]{27ae60}\textbf{\textcolor{white}{0.63}}
% \\

% CumRegret (low = good: green=low, red=high)
% Values: 13.68, 17.16, 18.90, 21.80, 36.00, 36.00, 37.99, 36.23, 22.41, 22.84, 16.61
CumRegret
  & \cellcolor[HTML]{27ae60}\textbf{\textcolor{white}{13.7}}
  & \cellcolor[HTML]{82ca60}\textbf{\textcolor{black}{17.2}}
  & \cellcolor[HTML]{a8d96a}\textbf{\textcolor{black}{18.9}}
  & \cellcolor[HTML]{f1c40f}\textbf{\textcolor{black}{21.8}}
  & \cellcolor[HTML]{e74c3c}\textbf{\textcolor{white}{36.0}}
  & \cellcolor[HTML]{e74c3c}\textbf{\textcolor{white}{36.0}}
  & \cellcolor[HTML]{c0392b}\textbf{\textcolor{white}{37.9}}
  & \cellcolor[HTML]{e74c3c}\textbf{\textcolor{white}{36.2}}
  & \cellcolor[HTML]{d4ac0d}\textbf{\textcolor{black}{22.4}}
  & \cellcolor[HTML]{d4ac0d}\textbf{\textcolor{black}{22.8}}
  & \cellcolor[HTML]{bee06a}\textbf{\textcolor{black}{16.6}}
\\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Heatmap of algorithm performance metrics. Colors follow a red--yellow--green diverging colormap (red = worst, yellow = middle, green = best). For MeanReward, MedianReward, K*MinFrac, BestArmFrac, higher is better; for SuffFailFreq($T$/2), GreedyFrac, CumRegret, lower is better. Columns $\tau \in \{0, 0.3, 0.7, 1, 1.5, 2\}$ correspond to a temperature parameter sweep. Dashes indicate metrics not applicable to that configuration.}
\end{table}
